Luminous Supernovae: Unveiling a Population Between Superluminous and Normal Core-collapse Supernovae

Stripped-envelope core-collapse supernovae can be divided into two broad classes: the common Type Ib/c supernovae (SNe Ib/c), powered by the radioactive decay of $^{56}$Ni, and the rare superluminous supernovae (SLSNe), most likely powered by the spin-down of a magnetar central engine. Up to now, the intermediate regime between these two populations has remained mostly unexplored. Here, we present a comprehensive study of 40 \textit{luminous supernovae} (LSNe), SNe with peak magnitudes of $M_r = -19$ to $-20$ mag, bound by SLSNe on the bright end and by SNe Ib/c on the dim end. Spectroscopically, LSNe appear to form a continuum between Type Ic SNe and SLSNe. Given their intermediate nature, we model the light curves of all LSNe using a combined magnetar plus radioactive decay model and find that they are indeed intermediate, not only in terms of their peak luminosity and spectra, but also in their rise times, power sources, and physical parameters. We sub-classify LSNe into distinct groups that are either as fast-evolving as SNe Ib/c or as slow-evolving as SLSNe, and appear to be either radioactively or magnetar powered, respectively. Our findings indicate that LSNe are powered by either an over-abundant production of $^{56}$Ni or by weak magnetar engines, and may serve as the missing link between the two populations.

==> mycommands.tex <==
% New Commands
\newcommand{\tc}[2][red]{\textcolor{#1}{\emph{\textbf{#2}}}}
\newcommand{\ksmag}{\emph{Ks}~magnitudes }
\newcommand{\jmag}{\emph{J}~magnitudes }
\newcommand{\kpmags}{\emph{Kp}~magnitudes }
\newcommand{\kpmag}{\emph{Kp}~magnitude }
\newcommand{\teff}{\ensuremath{T_{\mathrm{eff}}}}
\newcommand{\logg}{\ensuremath{\log g}}
\newcommand{\kepler}{{\em Kepler}\xspace}
\def\msun{{\rm\,M_\odot}}
\def\rsun{{\rm\,R_\odot}}
\def\mearth{{\rm\,M_\oplus}}
\def\rearth{{\rm\,R_\oplus}}
\def\fearth{{\rm\,F_\oplus}}
\def\lsun{{\rm\,L_\odot}}
\newcommand{\hho}{H$_2$O}
\newcommand{\hh}{H$_2$}
\newcommand{\oo}{O$_2$}
\newcommand{\chhhh}{CH$_4$}
\newcommand{\mjup}{{\rm M}_{\rm Jup}}
\newcommand{\kms}{\rm km\ s^{-1}}
\newcommand{\mps}{\rm m\ s^{-1}}
\newcommand{\cspg}{\rm\ cm^2\ g^{-1}}
\newcommand{\ergs}{\rm\ erg\ s^{-1}}
\newcommand{\kelvin}{\rm K}
\newcommand{\angstrom}{\rm \AA}
\newcommand{\oneday}{\rm day}
\newcommand{\days}{\rm days}
\newcommand{\hours}{\rm hours}
\newcommand{\meter}{\rm m}
\newcommand{\HST}{{\it HST}}
\newcommand{\hubble}{{\it HST}}
\newcommand{\spitzer}{{\it Spitzer}}
\newcommand{\fermi}{{\it Fermi}}
\newcommand{\swift}{{\it Swift}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\mosfit}{{\tt MOSFiT}}
\newcommand{\zeroth}{$0^{\rm th}$}
\newcommand{\first}{$1^{st}$}
\newcommand{\second}{$2^{nd}$}
\newcommand{\third}{$3^{rd}$}
\newcommand{\fourth}{$4^{th}$}
\newcommand{\e}{${\rm e^{-}}$}
\newcommand{\persecond}{${\rm s^{-1}}$}
\newcommand{\perpixel}{${\rm pixel^{-1}}$}
\newcommand{\divideoot}{{\tt divide-oot}}
\newcommand{\modelramp}{{\tt model-ramp}}
\newcommand{\chisq}{$\chi^2$}
\newcommand{\calwf}{{\tt calwf3}}
\newcommand{\rp}{$R_{p}$}
\newcommand{\rs}{$R_{\star}$}
\newcommand{\flt}{{\tt flt}}
\definecolor{orange}{rgb}{.8,0.4,0}
\newcommand{\question}[1]{\sffamily {\em {\color{orange} [#1]}}\normalfont}
\newcommand{\todo}[1]{\sffamily {\em {\color{orange} #1}}\normalfont}
\newcommand{\mad}{\rm MAD}
\newcommand{\Mej}{M_{\rm ej}}
\newcommand{\vej}{v_{\rm ej}}
\newcommand{\apx}{\ensuremath{\sim}}
\newcommand{\WFDD}{{\tt WFDD}}
\newcommand{\WFDM}{{\tt WFDM}}
\newcommand{\WFDR}{{\tt WFDR}}

% Alternate Itemize
\newcommand{\outline}[1]{
\todo{\begin{itemize}
#1
\end{itemize}}}

% AutoRef Stuff
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section}

\renewcommand*{\sectionautorefname}{Section} 
\renewcommand*{\subsectionautorefname}{Section} 

% Citation Alias
\defcitealias{LP98}{LP98}
\defcitealias{CowpBerger15}{CB15}

